Is Scaling Learned Optimizers Worth It? Evaluating The Value of VeLO's 4000 TPU Months

We analyze VeLO (versatile learned optimizer), the largest scale attempt to train a general purpose "foundational" optimizer to date. VeLO was trained on thousands of machine learning tasks using over 4000 TPU months with the goal of producing an optimizer capable of generalizing to new problems while being hyperparameter free, and outperforming industry standards such as Adam. We independently evaluate VeLO on the MLCommons optimizer benchmark suite. We find that, contrary to initial claims: (1) VeLO has a critical hyperparameter that needs problem-specific tuning, (2) VeLO does not necessarily outperform competitors in quality of solution found, and (3) VeLO is not faster than competing optimizers at reducing the training loss. These observations call into question VeLO's generality and the value of the investment in training it.

==> old_tables.tex <==
\begin{table}[h]
    \centering
    \caption{(NOT INCLUDING VELO SHORTER RUN) Performance profile scores for all baseline algorithms across workloads. Time-To-Result and Steps-To-Results are reported when fixing wall-clock time and steps respectively across train and validation targets. VeLO speedups are only observed on validation targets in the time-controlled experiments when VeLO runs for a conservative number of steps that fit on the wall-clock time. VeLO speedups are budget-dependent; hyperparameter sensitive.}
    \label{tab:performance_scores}
    \begin{tabular}{ccccc}
         \toprule
          & \multicolumn{2}{l}{\textbf{Train Scores}} & \multicolumn{2}{l}{\textbf{Validation Scores}} \\
         \cmidrule(l){2-3} \cmidrule(l){4-5}
          Optimizer & Time & Step & Time & Step \\
         \midrule
         NAdam & 0.24 & 0.00 & 0.00 & 0.22 \\
         NAdamW & 0.36 & 0.25 & 0.49 & 0.00 \\
         Adam & \textbf{1.00} & \textbf{0.88} & 0.24 & \textbf{0.50} \\
         Nesterov & 0.00 & 0.00 & 0.00 & 0.00 \\
         VeLO & 0.19 & 0.00 & \textbf{0.75} & 0.34 \\
         HeavyBall & 0.00 & 0.00 & 0.00 & 0.00 \\
         \bottomrule
    \end{tabular}
\end{table}

